Convergence Rates of Distributed Consensus over Cluster Networks: A Two-Time-Scale Approach

We study the popular distributed consensus method over networks composed of a number of densely connected clusters with a sparse connection between them. In these cluster networks, the method often constitutes two-time-scale dynamics, where the internal nodes within each cluster reach consensus quickly relative to the aggregate nodes across clusters. Our main contribution is to provide the rate of the distributed consensus method, which characterize explicitly the impacts of the internal and external graphs on the performance of this method. Our main result shows that this rate converges exponentially and only scales with a few number of nodes, which is relatively small to the size of the network. The key technique in our analysis is to consider a Lyapunov function which captures the impacts of different time-scale dynamics on the convergence of the method. Our approach avoids using model reduction, which is the typical way according to singular perturbation theory and relies on relatively simple definitions of the slow and fast variables. In addition, Lyapunov analysis allows us to derive the rate of distributed consensus methods over cluster networks, which is missing from the existing works using singular perturbation theory. We illustrate our theoretical results by a number of numerical simulations over different cluster networks.

==> prelim.tex <==
% \section{PRELIMINARIES}

% For a vector $x \in \mathbb{R}^N$, the euclidean norm is denotes as $||x||$. We use boldface for a matrix $\mathbf{M}$ and denote by $\|\Mbf\|$ its $2$-norm. In addition, we denote by $\sigma_{2}(\mathbf{M})$ the second smallest eigenvalue of $\mathbf{M}$. Also, we denote by $\mathbf{1}_{N}$ a vector in $\mathbb{R}^{N}$ whose entries are equal to $1$. \\
% When $\mathbf{P}$ is a diagonal matrix  with entries $\frac{1}{N_{\alpha}}$ as diagonal elements, the following inequalities hold,

% \begin{align}\label{eq:inequality_p}
%      N_{\min}\mathbf{I} \leq \mathbf{P} \leq N_{\max}\mathbf{I} 
% \end{align}

% Similarly we have 

% \begin{align}\label{eq:inequality_p_inv}
%      \frac{1}{N_{\max}}\mathbf{I} \leq \mathbf{P}^{-1} \leq \frac{1}{N_{\min}}\mathbf{I}.
% \end{align}
% Finally, we denote by $N_{\min}$ and $N_{\max}$, respectively, as 
% \begin{align}
% N_{\min} = \min_{\alpha} N_{\alpha},\quad N_{\max} = \max_{\alpha}N_{\alpha}. \label{notation:Nmin_max}   
% \end{align}


% For our analysis of the second term in \eqref{eq:inequality_p_inv} we consider that for any two vectors $x, y \neq 0$ and a scalar $\eta > 0$, the following inequality holds

% \begin{align}\label{eq:inequality_AMGM}
%     2x^{T}y \leq 2||x||||y|| \leq \eta ||x||^{2} + \frac{1}{\eta}||y||^{2}
% \end{align}
